Enhancement of laser-driven ion acceleration in non-periodic nanostructured targets

Using particle-in-cell simulations, we demonstrate an improvement of the target normal sheath acceleration (TNSA) of protons in non-periodically nanostructured targets with micron-scale thickness. Compared to standard flat foils, an increase in the proton cutoff energy by up to a factor of two is observed in foils coated with nanocones or perforated with nanoholes. The latter nano-perforated foils yield the highest enhancement, which we show to be robust over a broad range of foil thicknesses and hole diameters. The improvement of TNSA performance results from more efficient hot-electron generation, caused by a more complex laser-electron interaction geometry and increased effective interaction area and duration. We show that TNSA is optimized for a nanohole distribution of relatively low areal density and that is not required to be periodic, thus relaxing the manufacturing constraints.

==> befehle.tex <==
% Formatting rules for mathematical mode
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\bra}[1]{$\left|\, #1\, \right>$}
\newcommand{\ket}[1]{$\left<\, #1\, \right|$}
\newcommand{\V}[1]{\vec{#1}} % Vector
%\newcommand{\M}[1]{\mathbf{#1}} % Matrix
% Symbols for mathematical mode
%\newcommand{\var}{\mathrm{var}} % Varianz
\newcommand{\E}{\mathrm{E}} % Erwartungswert
\newcommand{\rmi}{\mathrm{i}} % imaginary unit
\newcommand{\rmd}{\mathrm{d}} % differential "d"
\newcommand{\FT}{\mathfrak{F}} % Fouriertransformation
\newcommand{\HT}{\mathfrak{H}} % Hilberttransformation
\newcommand{\DHT}{\mathfrak{DH}} % diskrete Hilberttransformation
\newcommand{\mad}{\mathrm{mad}} % nean average deviation
\newcommand{\rms}{\mathrm{rms}} % root mean square
\newcommand{\var}{\mathrm{var}} % variance
\newcommand{\cov}{\mathrm{cov}} % covariance
\newcommand{\tr}{\mathrm{tr}} % trace
\newcommand{\diag}{\mathrm{diag}} % trace
\newcommand{\D}{\mathrm{D}} % standard deviation
\newcommand{\cc}{\mrm{c}.\mrm{c}.} %conjugate complex of the left expression

%Mengen:
\newcommand{\N}{\mathbb{N}} % Natürliche Zahlen
\newcommand{\R}{\mathbb{R}} % reelle Zahlen
\newcommand{\C}{\mathbb{C}} % complexe Zahlen
\newcommand{\Q}{\mathbb{Q}} % rationale Zahlen
\newcommand{\M}{\mathbb{M}} % Menge M
\newcommand{\Z}{\mathbb{Z}} % ganze Zahlen
\newcommand{\Zi}{\mathbb{Z}[\rmi]} % ganze Zahlen
\newcommand{\I}{\mathbb{I}} % Indexmenge
\newcommand{\Lcal}{\mathcal{L}} % Lösungsmenge
\newcommand{\Ucal}{\mathcal{U}} % Lösungsmenge eines hom. Systems

%Logik:
\newcommand{\und}{\wedge} % logisches und
\newcommand{\oder}{\vee} % logisches oder
\newcommand{\darausfolgt}{\Rightarrow} % daraus folgt
\newcommand{\darausfolgtr}{\Leftarrow} % daraus folgt rückwärts
\newcommand{\aqui}{\Leftrightarrow} % aquivalent
\newcommand{\hin}{\glqq\Rightarrow\grqq{}} % "daraus folgt"
\newcommand{\her}{\glqq\Leftarrow\grqq{}} % "daraus folgt rückwärts"

%Mathematische Funktionen:
\newcommand{\ggT}{\mbox{ggT}} % größter gemeinsamer Teiler
\newcommand{\modulo}{\mbox{ mod }}
\newcommand{\rect}{\mbox{rect}} % Rechteckfkt.
\newcommand{\ramp}{\mbox{ramp}} % Rechteckfkt.


%Physikalische Groessen:
\newcommand{\iotavec}{\mathbf{\iota}}
\newcommand{\avec}{\mathbf{a}}
\newcommand{\Avec}{\mathbf{A}}
\newcommand{\Vvec}{\mathbf{V}}
\newcommand{\Qvec}{\mathbf{Q}}
\newcommand{\Svec}{\mathbf{S}}	%Poynting vektor
\newcommand{\Fvec}{\mathbf{F}}	%flux vektor
\newcommand{\Evec}{\mathbf{E}}	%el.Feld
\newcommand{\Dvec}{\mathbf{D}}	%dielectische Verschiebung
\newcommand{\Hvec}{\mathbf{H}}	%mag.Feld
\newcommand{\Bvec}{\mathbf{B}}	%mag.Induktion
\newcommand{\Jvec}{\mathbf{J}}	%Strom
\newcommand{\rhovec}{\mathbf{\rho}}	%el.Feld
\newcommand{\Wvec}{\mathbf{W}}
\newcommand{\Pvec}{\mathbf{P}}	%Polarisation
\newcommand{\pvec}{\mathbf{p}}	%Polarisation
\newcommand{\xvec}{\mathbf{x}}  %Ortsvektor
\newcommand{\uvec}{\mathbf{u}}  %Ortsvektor
\newcommand{\wvec}{\mathbf{w}}
\newcommand{\rvec}{\mathbf{r}}
\newcommand{\vvec}{\mathbf{v}}  %Ortsvektor.
\newcommand{\jvec}{\mathbf{j}}	%el.Strom
\newcommand{\dvec}{\mathbf{d}}	%mag.Feld
\newcommand{\bvec}{\mathbf{b}}  %mag.Induktion
\newcommand{\evec}{\mathbf{e}}	%el.Feld
\newcommand{\hvec}{\mathbf{h}}	%mag.Feld#
\newcommand{\fvec}{\mathbf{f}}
\newcommand{\gvec}{\mathbf{g}}
\newcommand{\kvec}{\mathbf{k}}
\newcommand{\nvec}{\mathbf{n}}
\newcommand{\Ivec}{\mathbf{I}}
\newcommand{\Cvec}{\mathbf{C}}

%Nummerierung:
\newcommand{\zeroth}{$0^{\text{th}}\,$}
\newcommand{\first}{$1^{\text{st}}\,$}
\newcommand{\second}{$2^{\text{nd}}\,$}
\newcommand{\third}{$3^{\text{rd}}\,$}
\newcommand{\fourth}{$4^{\text{th}}\,$}

\DeclareSymbolFont{lettersA}{U}{txmia}{m}{it}
\DeclareMathSymbol{\real}{\mathord}{lettersA}{"92} % real numbers
\DeclareMathSymbol{\cplx}{\mathord}{lettersA}{"83} % complex numbers

% Schelm's special command to mark passages needing rework:
\newcommand{\yuck}[1]{\marginpar{\raggedright \tiny {\bf YUCK:}\\ #1}}
  
%%% Local Variables: 
%%% mode: latex
%%% mode: auto-fill
%%% TeX-master: "document"
%%% End: 

